Uniform Bounds for Scheduling with Job Size Estimates

We consider the problem of scheduling to minimize mean response time in M/G/1 queues where only estimated job sizes (processing times) are known to the scheduler, where a job of true size $s$ has estimated size in the interval $[\beta s, \alpha s]$ for some $\alpha \geq \beta > 0$. We evaluate each scheduling policy by its approximation ratio, which we define to be the ratio between its mean response time and that of Shortest Remaining Processing Time (SRPT), the optimal policy when true sizes are known. Our question: is there a scheduling policy that (a) has approximation ratio near 1 when $\alpha$ and $\beta$ are near 1, (b) has approximation ratio bounded by some function of $\alpha$ and $\beta$ even when they are far from 1, and (c) can be implemented without knowledge of $\alpha$ and $\beta$? We first show that naively running SRPT using estimated sizes in place of true sizes is not such a policy: its approximation ratio can be arbitrarily large for any fixed $\beta < 1$. We then provide a simple variant of SRPT for estimated sizes that satisfies criteria (a), (b), and (c). In particular, we prove its approximation ratio approaches 1 uniformly as $\alpha$ and $\beta$ approach 1. This is the first result showing this type of convergence for M/G/1 scheduling. We also study the Preemptive Shortest Job First (PSJF) policy, a cousin of SRPT. We show that, unlike SRPT, naively running PSJF using estimated sizes in place of true sizes satisfies criteria (b) and (c), as well as a weaker version of (a).

==> figures/tikz-macros.tex <==
\makeatletter

% Prelude sets $ to active, but calc needs it as math shift.
\catcode`\$=3 % math shift

\usetikzlibrary{backgrounds, math, shapes, shapes.arrows, positioning,
  decorations.markings, decorations.pathreplacing, calligraphy}

\tikzset{
  bgbox/.style={framed, background rectangle/.style={fill=black!7, rounded corners=1em}},
  figure/.style={x=\xscale, y=\yscale, semithick, font=\footnotesize, bgbox},
  axis/.style={thin},
  guide/.style={thin, black!30, dashed},
  srpt-b/.style={ultra thick, color=orange!60!yellow!80!black},
  srpt-se/.style={ultra thick, color=cyan!75!blue!90!white},
  psjf-e/.style={ultra thick, color=green!40!yellow!70!black},
  srpt-e/.style={ultra thick, color=magenta!55!blue!75!white},
  psjf/.style={ultra thick, color=green!60!blue!85!black},
  srpt/.style={ultra thick, color=magenta!60!red!85!black},
  size/.style={ultra thick, color=magenta!88!blue!95!white},
}

\def\@above{above}
\def\@below{below}
\def\@negative{-}
\newcommand{\downmode}{%
  \def\@above{below}
  \def\@below{above}
  \def\@negative{}}

\newcommand{\xscale}{7}
\newcommand{\yscale}{7}
\newcommand{\ticksize}{3}
\newcommand{\arrowsize}{5}
\newcommand{\xarrowsize}{(\arrowsize/\xscale)}
\newcommand{\yarrowsize}{(\arrowsize/\yscale)}

\newcommand{\projx}[1]{($ (0,0)!#1!(1,0) $)}
\newcommand{\projxheight}[2]{($ (0,#2)!#1!(1,#2) $)}
\newcommand{\midpt}[2]{($ #1!0.5!#2 $)}

\newcommand{\xguide}[3][]{%
  \draw[axis] ({#2}, 0) -- ({#2}, {\@negative(\ticksize)/\yscale})
  node[\@below] {\ifempty{#1}{$#2$}{#1}\vphantom{by}};
  \draw[guide] ({#2}, 0) -- ({#2}, {#3});}
\newcommand{\yguide}[3][]{%
  \draw[axis] (0, {#3}) -- (-\ticksize/\xscale, {#3})
  node[left] {\ifempty{#1}{$#3$}{#1}};
  \draw[guide] (0, {#3}) -- ({#2}, {#3});}
\newcommand{\yguidenolabel}[2]{%
  \draw[guide] (0, {#2}) -- ({#1}, {#2});}

\newcommand{\axes}[6]{%
  \draw[axis, ->] (-\ticksize/\xscale, 0)
  node[left] {#3\vphantom{by}} -- ({#1 + \xarrowsize}, 0) node[right] {#4\vphantom{by}};
  \draw[axis, ->] (0, \@negative\ticksize/\yscale)
  node[\@below] {#5\vphantom{by}} -- (0, {#2 + \yarrowsize})
  node[\@above] {#6\vphantom{by}};}

% Set $ back to active for prelude
\catcode`\$=13 % active
\makeatother

